Conformal Computing: Algebraically connecting the hardware/software boundary using a uniform approach to high-performance computation for software and hardware applications

We present a systematic, algebraically based, design methodology for efficient implementation of computer programs optimized over multiple levels of the processor/memory and network hierarchy. Using a common formalism to describe the problem and the partitioning of data over processors and memory levels allows one to mathematically prove the efficiency and correctness of a given algorithm as measured in terms of a set of metrics (such as processor/network speeds, etc.). The approach allows the average programmer to achieve high-level optimizations similar to those used by compiler writers (e.g. the notion of "tiling"). The approach presented in this monograph makes use of A Mathematics of Arrays (MoA, Mullin 1988) and an indexing calculus (i.e. the psi-calculus) to enable the programmer to develop algorithms using high-level compiler-like optimizations through the ability to algebraically compose and reduce sequences of array operations. Extensive discussion and benchmark results are presented for the Fast Fourier Transform and other important algorithms.

==> axbx.tex <==
\begin{verbatim}

      010101010101010101010101010101010101010101010101
      001100110011001100110011001100110011001100110011
      000011110000111100001111000011110000111100001111
 axbx 000000001001010010011011100100101101110110111111
 0000  a     b                 c     d
 0001    a     b                 c     d
 0010  e     f                 g     h
 0011    e     f                 c     d
 0100             a     b                 c     d
 0101                a     b                 c     d
 0110             e     f                 g     h
 0111                e     f                 g     h
 1000  i     j                 k     l
 1001     i     j                 k     l
 1010  m     n                 o     p
 1011     m     n                 o     p
 1100              i     j                 k     l
 1101                 i     j                 k     l
 1110              m     n                 o     p
 1111                 m     n                 o     p

\end{verbatim}


==> macros.tex <==
\addtolength{\oddsidemargin}{-.55in}
\addtolength{\textwidth}{1.1in}
\addtolength{\topmargin}{-.84in}
\addtolength{\textheight}{1.2in} 
\newcommand{\cat}{+\!\!\!\!+}
%\newcommand{\cat}{\mbox{$+\!\!+_s$}}
\newcommand{\Take}{\mbox{Take}}
\newcommand{\take}{\,\bigtriangleup\,}
\newcommand{\Drop}{\mbox{Drop}}
\newcommand{\drop}{\,\bigtriangledown\,}
\newcommand{\rshp}{\,\widehat{\Rho}\;}
\newcommand{\Rho}{\,\rho\,}
\newcommand{\Tau}{\,\tau\,}
\newcommand{\Dim}{\,\delta\,}
\newcommand{\transpose}{\bigcirc\!\!\!\!\!\backslash\;}

\newcommand{\Ravel}{\,\mbox{\tt rav}\,}
\newcommand{\Gradeup}{\,\mbox{\tt gu}\,}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{theorem}{Theorem}


==> text1.tex <==

We present a systematic, algebraically based, design methodology for efficient
implementation of computer programs optimized over multiple levels of the 
processor/memory and network hierarchy.  Using a common formalism to 
describe the problem and the partitioning of data over processors and memory 
levels allows
one to mathematically prove the efficiency and correctness of a given algorithm
as measured in terms of a set of metrics (such as processor/network speeds, 
etc.).  The approach allows the average programmer to achieve high-level
optimizations similar to those used by compiler writers (e.g. the notion of 
{\em tiling}).

The approach is similar in spirit to other efforts using libraries of 
algorithm building blocks based on C++ template classes. In POOMA for example,
expression templates using the Portable Expression Template Engine (PETE) 
\break (http://www.acl.lanl.gov.pete)
were used to achieve efficient distribution of array indexing over scalar
operations~\cite{Humphrey97,Karmesin98,Vlot:1991:PA,Wester:1991:POS,Pooma96,musser,austern,weiss,reynders,veldhuizen}. 

As another example, The Matrix Template 
Library (MTL) \cite{lumsdaine97,lumsdaine98} is a system that handles dense 
and sparse matrices, and uses template meta-programs to generate tiled 
algorithms for dense matrices.

 For example:

\begin{equation}
(A + B)_{ij} = A_{ij} + B_{ij},
\end{equation}
can be generalized to the situation in which the multi-dimensional 
arrays $A$ and $B$ are selected using a vector of indices $\vec v$.

In POOMA $A$ and $B$ were represented as classes and expression templates
were used as re-write rules to efficiently carry out the translation 
to scalar operations implied by:

\begin{equation}
(A + B)_{\vec v} = A_{\vec v} + B_{\vec v}
\label{traditional}
\end{equation}

The approach presented in this paper makes use of A Mathematics of Arrays (MoA)
and an indexing calculus (i.e. the $\psi$ calculus) to enable the programmer
to develop algorithms using high-level compiler-like optimizations through
the ability to algebraically compose and reduce sequences of array operations.

As such, the translation from the left hand side of Eq.~\ref{traditional}
to the right side is just one of a wide variety of operations that can 
be carried out using this algebra.  In the MoA formalism, the array
expression in Eq.~\ref{traditional} would be written:

\begin{equation}
{\vec v} \psi (A + B) = {\vec v} \psi A + {\vec v} \psi B
\end{equation}
where we have introduced the {\em psi-operator} $\psi$ to denote the 
operation of extracting an element from the multi-dimensional array using
the index vector (${\vec v}$).

In this paper we give a demonstration of the approach as applied to the 
creation of efficient implementations of the Fast Fourier Transform (FFT) 
optimized
over multi-processor, multi-memory/network, environments.  Multi-dimensional
data arrays are {\em reshaped} through the process of {\em dimension lifting}
to explicitly add dimensions to enable indexing blocks of data over
the various levels of the hierarchy.  A sequence of array operations 
(represented by the various operators of the algebra acting on arrays)
is algebraically composed to achieve the {\em Denotational Normal Form} (DNF).
Then the $\psi$-calculus is used to reduce the DNF to the ONF ({\em Operational
Normal Form}) which explicitly expresses the algorithm in terms of loops
and operations on indices.  The ONF can thus be directly translated into
efficient code in the language of the programmer's choice be it for hardware
or software application.

The application we use as a demonstration vehicle -- the Fast Fourier 
Transform -- is of significant interest in its own right. 
The Fast Fourier Transform (FFT) is one of the most
important computational algorithms and its use is pervasive in science and
engineering. The work in this paper is a companion to two previous
papers~\cite{papers12} in which the FFT was optimized in terms of in-cache
operations leading to factors of {\em two} to {\em four} speedup in comparison
with our previous records.  Further background material including
comparisons with library routines can be found in
Refs.~\cite{lenss3,lenss4,mullin.small:,mul03} and~\cite{cpc}.

Our algorithm can be seen to be a generalization of similar work aimed at
out-of-core optimizations~\cite{cormen}. Similarly, block decompositions
of matrices (in general) are special cases of our {\em rehape-traspose} design.
Most importantly, our designs are general for any partition size,
i.e. not necessary blocked in squares, and any number of dimensions.
Furthermore, our designs use linear transformations from an algebraic
specification and thus they are {\bf verified}. Thus, by specifying
designs (such as Cormen's and others~\cite{cormen}) using these 
techniques, these designs too could be verified.

The purpose of this paper {\bf IS NOT} to attempt any serious analysis of the
number of cache misses incurred by the algorithm in the spirit of
of Hong and Kung and others~\cite{hongkung,savage,vitter93algorithms}.
Rather, we  present an {\bf algebraic} method
that achieves (or is competitive) with such  optimizations
{\bf mechanically}. Through linear transformations we
produce a  {\bf normal form}, the ONF, that is directly implementable in any
hardware or software language and is realized in any of the processor/memory
levels~\cite{fftharry}.
Most importantly, our designs are completely general in that through {\bf
dimension lifting} we can produce any number of levels in the processor/memory
hierarchy.

One objection to our approach is that one might incur an unacceptable
performance cost due to the periodic rearrangement of the data that is often 
needed.  This will
not, however, be the case if we  pre-fetch data before
it is needed.  The necessity to pre-fetch data also exists in other
similar cache-optimized schemes.  Our algorithm does what the
compiler community calls {\em tiling}. Since we have analyzed the loop
structures,  access patterns, and speeds of the processor/memory levels,
pre-fetching becomes a deterministic cost function that can easily
be combined with  {\em reshape-transpose} or {\em tiling} operations.

Again we make no attempt to optimize the algorithm for any particular
architecture.  We provide a general algorithm in the form of an Operational
Normal Form that allows the user to specify the blocking size at run time.
This ONF therefore enables the individual user to choose the blocking
size that gives the best performance for any individual machine, assuming
this intentional information can be processed by a compiler\footnote{Processing intentional information will be the topic of a future
paper}.

It is also important to note the importance of running {\em reproducible
 and deterministic} experiments. Such experiments are only possible
when dedicated resources exist {\em AND} no interrupts or randomness effects
memory/cache/communications behavior. This means that multiprocessing
and time sharing must be turned off for both OS's and Networks.

Conformal Computing\footnote{The name
Conformal Computing \copyright $\;$ is protected.  Copyright 2003,
The Research Foundation of State University of New York, University at Albany.}
 is the name given by the authors to this algebraic approach 
to the construction of computer programs for array-based computations in science
and engineering. The reader should not be misled by the name.  Conformal in
this sense is not related to {\em Conformal Mapping} or similar constructs
from mathematics although it was inspired by these concepts in which
certain properties are preserved under transformations.  In particular,
by {\em Conformal Computing} we mean a mathematical system that {\it conforms}
as closely as possible to the underlying structure of the hardware.
Further details of the theory including discussion of MoA and $\psi$-calculus
are provided in the appendix.
 

